Optimal Clustering from Noisy Binary Feedback

We study the problem of clustering a set of items from binary user feedback. Such a problem arises in crowdsourcing platforms solving large-scale labeling tasks with minimal effort put on the users. For example, in some of the recent reCAPTCHA systems, users clicks (binary answers) can be used to efficiently label images. In our inference problem, items are grouped into initially unknown non-overlapping clusters. To recover these clusters, the learner sequentially presents to users a finite list of items together with a question with a binary answer selected from a fixed finite set. For each of these items, the user provides a noisy answer whose expectation is determined by the item cluster and the question and by an item-specific parameter characterizing the {\it hardness} of classifying the item. The objective is to devise an algorithm with a minimal cluster recovery error rate. We derive problem-specific information-theoretical lower bounds on the error rate satisfied by any algorithm, for both uniform and adaptive (list, question) selection strategies. For uniform selection, we present a simple algorithm built upon the K-means algorithm and whose performance almost matches the fundamental limits. For adaptive selection, we develop an adaptive algorithm that is inspired by the derivation of the information-theoretical error lower bounds, and in turn allocates the budget in an efficient way. The algorithm learns to select items hard to cluster and relevant questions more often. We compare the performance of our algorithms with or without the adaptive selection strategy numerically and illustrate the gain achieved by being adaptive.

==> Declarations.tex <==


\section*{Declarations}

\paragraph{Funding}
This research is partly funded by 
\updated{the} Nakajima Foundation Scholarship, 
Vetenskaprådet, 
Institute of Information \& communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government (MSIT) (No.2019-0-00075, Artificial Intelligence Graduate School Program (KAIST) and No.2019-0-01906, Artificial Intelligence Graduate School Program (POSTECH)),
\updated{and
JSPS KAKENHI Grant No.~23K19986.
}


\paragraph{Conflicts of interest/Competing interests}
Not applicable.


\paragraph{Availability of data and material}
We have attached the data used and generated raw data at the following URL: https://bit.ly/3Am5DhX


\paragraph{Code availability}

We have attached the source code at the following URL: https://bit.ly/3Am5DhX

\paragraph{Ethics approval}

Not applicable.

\paragraph{Consent to participate}

Not applicable.


\paragraph{Consent for publication }

Not applicable.


==> app_algorithm2.tex <==

\section{Adaptive Clustering Algorithm} 


\begin{algorithm}
	\caption{Adaptive Clustering Algorithm. }
	\label{alg:adaptive_sampling}
	\begin{algorithmic}
		\STATE \textbf{Input: } $K$, $T$
		\STATE \textbf{Initialization: } $\tau \gets \left\lfloor {T} /\left( 4 \log\left(\frac{T}{n}\right) \right)\right\rfloor$
		\STATE $\hat{p}_{k \ell } \gets 0 $ for all $\ell \in [L], k \in [K]$
		\STATE $\hat{h}_i \gets 0.5$ for all $i \in \set{I}$
		\WHILE {$t < T$}
		\STATE $ Y_{i \ell} \gets \sum_{t'=1}^t \mathbbm{1}[i \in \set{W}_{t'}, \ell_{t'}= \ell]$
		\STATE $\hat{q}_{i \ell} \gets \frac{\sum_{t'=1}^t \mathbbm{1}[i \in \set{W}_{t'}, \ell_{t'}= \ell, X_{i \ell t'} = 1]}{Y_{i \ell}} $ if $Y_{i \ell}>0$, $\frac{1}{2}$ otherwise
		\IF {\textnormal{mod}$(t, \tau) = 0$}
		\STATE Use \text{Algorithm~\ref{alg:kmeans_for_r}} with input $K, t$ to  obtain the estimated clusters $\{\set{S}_k\}_{k = 1,\ldots,K}$
		\STATE {\bf Estimate statistical parameters:}
		\STATE	 $\hat{p}_{k \ell } \gets  \frac{1}{2} \left( \frac{\sum_{i \in \set{S}_k} (2 \hat{q}_{i \ell} - 1)}{|\set{S}_k|} + 1\right)$ 
		for all $\ell \in [L], k \in [K]$		
		\STATE { $\hat{h}_i \gets 
			\max\left\{0.5, \argmin_{h' \in [1/2, 1]} \left\{ \sum_{\ell \in [L]} Y_{i \ell} \KL (h' \hat{p}_{\hat{\sigma}(i) \ell} +\bar{h'} \bar{ \hat{p}}_{\hat{\sigma}(i) \ell}, \hat{q}_{i \ell}) \right\} - \sqrt{\frac{\log(t)}{ 10 \sum_{\ell } Y_{i \ell}}} \right\},$ 
		}
		\STATE for all $i \in \set{I}$ 
		\ENDIF
		\STATE {\bf Adaptive item question selection:} 
		\STATE $i^\star \gets \argmin_{i \in \set{I}} \hat{d}_i$	where $\hat{d}_{i} =  {d}_{i}(h'_i, k'_i, \vec{Y})$,
		\STATE where	$k'_{i} = \argmin_{k' \neq \hat{\sigma}(i)} \min_{h' \in [1/2, 1]} {d}_{i}(h', k',\vec{Y})$,
		\STATE $h'_{i} =  \argmin_{h' \in [1/2, 1]} {d}_{i}(h', k'_i, \vec{Y})$, 
		\STATE and ${d}_{i}(h', k', \vec{Y})
		= \sum_{\ell =1}^L Y_{i\ell} \KL ( 
		{h}' \hat{p}_{k' \ell}+\bar{{h}}' \bar{\hat{p}}_{k'\ell}, \hat{h}_i\hat{p}_{\hat{\sigma}(i) \ell}+\bar{\hat{h}}_i \bar{\hat{p}}_{\hat{\sigma}(i)\ell}) .$
		\STATE $\ell^\star \gets \argmax_{\ell} \min_{k' \neq \hat{\sigma}(i^\star)} 
		\KL(h'_{i^\star} \hat{p}_{k' \ell}  + h'_{i^\star} \bar{\hat{p}}_{k' \ell}, \hat{h}_{i^\star} \hat{p}_{\hat{\sigma}(i^\star) \ell} +\bar{\hat{h}}_{i^\star} \bar{\hat{p}}_{\hat{\sigma}(i^\star) \ell} ) $.
		\STATE Present items $\set{W}_t$ (including $i^\star$) with the smallest $\hat{d}_i$ with question $\ell^\star$.
		\ENDWHILE
		\STATE {\bf Output:}  $\{\set{S}_k\}_{k \in [K]}$
	\end{algorithmic}
\end{algorithm}


The adaptive (item, question) selection algorithm is described in Algorithm \ref{alg:adaptive_sampling}. 
In order to reduce the computational complexity of the algorithm, we replace the KL function in the definition of  ${d}_i$ by a simple quadratic function (as suggested in Proposition~\ref{prop:bound-D-M}). This simplifies the minimization problem over $h'$ to find $h_i'$. We actually have an explicit expression for $h_i'$ with this modification.

\paragraph{Computing infrastructure and code submission.}
The simulations were performed on a desktop computer with Intel Core i7-8700B 3.2 GHz CPU and 32 GB RAM. 
